X-SRL: A Parallel Cross-Lingual Semantic Role Labeling Dataset

Even though SRL is researched for many languages, major improvements have mostly been obtained for English, for which more resources are available. In fact, existing multilingual SRL datasets contain disparate annotation styles or come from different domains, hampering generalization in multilingual learning. In this work, we propose a method to automatically construct an SRL corpus that is parallel in four languages: English, French, German, Spanish, with unified predicate and role annotations that are fully comparable across languages. We apply high-quality machine translation to the English CoNLL-09 dataset and use multilingual BERT to project its high-quality annotations to the target languages. We include human-validated test sets that we use to measure the projection quality, and show that projection is denser and more precise than a strong baseline. Finally, we train different SOTA models on our novel corpus for mono- and multilingual SRL, showing that the multilingual annotations improve performance especially for the weaker languages.

==> tables/special_cases.tex <==
\begin{table*}
\centering

\begin{tabularx}{\linewidth}{cL}
\toprule
\multirow{2}{*}{1} & 

\scriptsize{The account had \textbf{billed} about \$6 million in 1988, according to Leading National Advertisers.}                                                                                                                          \\
                   & \scriptsize{Das Konto hatte 1988 etwa 6 Millionen Dollar \textbf{in Rechnung gestellt}, so die Leading National Advertisers.}                                                                                                  \\ \midrule
                   
\multirow{2}{*}{2} & \scriptsize{People aren't \textbf{panicking}.}                                                                                                                                                        \\
                   & \scriptsize{La gente no está \textbf{entrando en pánico}.}                                                                                                                                              \\ \midrule
                   
\multirow{2}{*}{3} & \scriptsize{The economy does, however , \textbf{depend} on the confidence of businesses, consumers and foreign investors .}                                                                                                                                                \\
                   & \scriptsize{Die Wirtschaft \textbf{hängt} jedoch vom Vertrauen von Unternehmen, Verbrauchern und ausländischen Investoren \textbf{ab}.} \\ \midrule
                   
\multirow{2}{*}{4} & \scriptsize{But while the \textbf{New York Stock Exchange} did n't fall apart Friday as the \textbf{Dow Jones Industrial Average} plunged 190.58 points.}                  \\
                   & \scriptsize{Mais si la \textbf{Bourse de New York} ne s' est pas effondrée vendredi alors que le \textbf{Dow Jones Industrial Average} a chuté de 190,58 points.} \\ \midrule
\multirow{2}{*}{5} & \scriptsize{\textbf{I} think at this point \textbf{we} want to be a lot more efficient.}                                                                                                                                                                    \\
                   & \scriptsize{\textbf{X} Creo que en este momento \textbf{X} queremos ser mucho más eficientes .}                                                                                                                                                             \\ \bottomrule
\end{tabularx}

\caption{\label{tab:special_cases}
Special Cases Caption
}
\end{table*}
